Distributed Subweb Specifications for Traversing the Web

Link Traversal-based Query Processing (ltqp), in which a sparql query is evaluated over a web of documents rather than a single dataset, is often seen as a theoretically interesting yet impractical technique. However, in a time where the hypercentralization of data has increasingly come under scrutiny, a decentralized Web of Data with a simple document-based interface is appealing, as it enables data publishers to control their data and access rights. While ltqp allows evaluating complex queries over such webs, it suffers from performance issues (due to the high number of documents containing data) as well as information quality concerns (due to the many sources providing such documents). In existing ltqp approaches, the burden of finding sources to query is entirely in the hands of the data consumer. In this paper, we argue that to solve these issues, data publishers should also be able to suggest sources of interest and guide the data consumer towards relevant and trustworthy data. We introduce a theoretical framework that enables such guided link traversal and study its properties. We illustrate with a theoretic example that this can improve query results and reduce the number of network requests. We evaluate our proposal experimentally on a virtual linked web with specifications and indeed observe that not just the data quality but also the efficiency of querying improves. Under consideration in Theory and Practice of Logic Programming (TPLP).

==> proofs.tex <==

\begin{proposition}
    \ldql captures distribution of constant source selectors. %functions. 
\end{proposition}
\begin{proof}
    Let $\sselect$ be any constant function $\allwolds\to2^\uris$ and let $U$ be the image of any \WOLD under $\sselect$. Let $a$ be a fresh \URI; we define $\enc(\sselect)$ to be the set of triples $\{\triple{a}{a}{u}\mid u\in U\}$. For $\lpemeta$ we take $(a,a,\_)^*$. This indeed expresses to follow every link as indicated by the constant function; it is not hard to see that in this case the correspondence indeed holds.
    %  Consider the encoding of the constant function that maps every 
\end{proof}

\bart{the following two lemmas are guesses. We don't really need them. But might be useful to udnerstand limits of expressability more}

\begin{lemma}
 If $(\enc,\lpemeta)$ \emph{captures} $\classS$, then so does $(\enc,(\lpemeta)^*)$. 
\end{lemma}
\begin{proof}
 \bart{This is a guess. To be verified. }
\end{proof}


\begin{lemma}
If \ldql captures distribution of $\classS_1$ and of $\classS_2$, then it also captures distribution of $\classS_1\cup \classS_2$.  
\end{lemma}
\begin{proof}
 \bart{Not hundred percent sure, but my guess is this would hold. We would assume the encodings use distinct predicates and then use the meta lpe. $({\lpemeta}_1 + {\lpemeta}_2 )^*$.} 
\end{proof}

In the next two propositions, we will make use of the following source selectors for identifying documents of interest: 
\[\mathit{all}_{p,u}: \wold \mapsto \lpeEval{(+,p,\_)^*}{\wold}{\uri}.\]
Intuitively, the function $\mathit{all}_{p,u}$ identifies the set of all $p$s of $p$s of .... of $u$. For instance, by taking $p = \mathit{friend}$, we include all direct or indirect friends of $u$. By taking $p = \mathit{trust}$, we get all \URI{}s trusted by the publisher of $u$ (or trusted by those or ...). 

The first proposition states that when $p$ is fixed, i.e., when all data publishers use the same type of inclusion property, \ldql can capture this. However, in \cref{prop:inexp}, we show that when every agent is allowed to choose a different $p$, this can no longer be captured. 
\todo{something about the fact that is a realistic scenario}
% \todo{introduce and explain the functions before proposition}

To help prove our proposition bout inexpensiveness, we shall show some property of \lpes. Namely, we say that two triples \tuple{t_1, t_2,t_3} and \tuple{t_1', t_2',t_3'} in context $u$ are indistinguishable by a pure \lpe $e$ if for $i\in \brak{1,2,3}$
\begin{itemize}
	\item $t_i=t_i'=u$, or
	\item $t_i$ and $t_i'$ do not occur in $e$, or
	\item $t_i$ occurs in $e$ and $t_i'=t_i$
\end{itemize}

\begin{lemma}
	If an \lpe $e$ yields $u_1$ by matching a triple \tuple{t_1, t_2,u_1} in context $u$ and \tuple{t_1', t_2',u_2} and \tuple{t_1, t_2,u_1} are indistinguishable by $e$ in context $u$, and $u_1$ and $u_2$ are bi-similar\todo{not defined yet}, then $e$ yields $u_2$.
\end{lemma}

\begin{proof}
	From the fact that \tuple{t_1', t_2',u_2} and \tuple{t_1, t_2,u_1} are indistinguishable by $e$ in context $u$, we can consider only three cases for $t_i$ and $t_i'$ for $i\in \brak{1,2}$
	\begin{itemize}
		\item $t_i=u$, but then $t_i'=u$,
		\item $t_i$ and $t_i'$ do not occur in $e$, but then the only way for $e$ to match them is using the $\_$ placeholder which match both of them,
		\item $t_i$ occurs in $e$, and then $t_i'=t_i$.
	\end{itemize}

	Moreover, because $u_1$ and $u_2$ are bi-similar and $u_1$ and $u_2$ do not occur in $e$, all \lpes of the form $[l]$ give a non empty result when evaluated in both $u_1$ and $u_2$\todo{seems to be developed further the idea of [l]}, then \tuple{t_1, t_2,u_1} can be substituted by  \tuple{t_1', t_2',u_2} and $u_2$ takes the place of $u_1$, thus $e$ yields $u_2$ as well. \younes{rough version}
\end{proof}

\begin{proposition}
 Let $p$ be any \URI and let $\classS_p$ be the set of source selectors $\mathit{all}_{p,u}$ with $u\in \uris$.
 LDQL captures distribution of $\classS_p$.
\end{proposition}
\begin{proof}
This is shown using the encoding $\enc(\mathit{all}_{p,u})= \{\triple{a}{a}{u}\}$ and $\lpemeta = ((a,a,\_)/(+,p,\_)^*)^*$. 
Indeed, consider evaluation of this expression a \URI $u$. If $\data(\adoc(u))$ does \emph{not} contain triples matching $(a,a,\_)$ and hence the subweb construction of $\adoc(u)$ is empty. Otherwise, for each triple $(a,a,u')$ in $\data(\adoc(u))$, the link pattern $(a,a,\_)$ follows the link to $u'$. From there on, the pattern $(+,p,\_)$ instructs to include all $p$s of $p$s ... 
    The outermost star ensures that for each \uri that is found, also their subweb of interest is included.  
\end{proof}


\begin{proposition}\label{prop:inexp}
 Let $\classS_{\mathit{all}}$ be the set of all source selectors $p_u$ that map $\wold$ to $\lpeEval{(+,p,\_)^*}\wold\uri$. 
 LDQL \textbf{does not} capture distribution of $\classS_{\mathit{all}}$.
\end{proposition}
\begin{proof}
 Assume towards a contradiction that such an $\lpemeta$ and $\enc$ exist. Let $p$, $q$, $u_1, \dots ,u_4$ be \URIs that do not occur in  $\lpemeta$ and let $\ctxwold$ be the \caWOLD with $\docs = \{d_1,\dots, d_4\}$, $\adoc(u_i)=d_i$ for $i\in 1,\dots,4$, and 
 \[\data(d_1) = \{(u_1,p,u_2)\}, \data(d_2)= \{(u_2,p,u_3),(u_2,q,u_4)\}, \data(d_3)=\data(d_4)=\emptyset\]
 with construction $\ctx_{d_1}=\{(\mathit{all}_{p,u_1},\ltrue,\id)\}$ and $\ctx_{d_i}=\emptyset$ for $i>1$. This \caWOLD is 
visualized in \cref{fig:ex}. In this example \WOLD, clearly $\soi(d_1,\ctxwold) = \{d_1, d_2, d_3\}$. It is also clear that $\enc(\wold)$ only differs from $\wold$ in the data of $d_1$. 
Now, for \emph{any} \lpe $e$ that does not mention $p$ nor $q$ (and in particular, for any subexpression of $\lpemeta$), $u_3\in \lpeEval{e}{\wold}{u_2}$ if and only if $u_4\in \lpeEval{e}{\wold}{u_2}$ \younes{I find this argument natural and trivial. But in my case (if it is me who is proving the proposition), I would be skeptical in the sense that it is not sufficient and it should be proven further.} (and the same thus holds for $\enc(\wold)$). 
Since all the facts, it also follows that \younes{Same here. I would look to show why does it follow. Even though it is clear for me.} $d_3\in \lpeEval{\lpemeta}{\enc(\ctxwold)}{u_1}$ if and only if $d_4 \in \lpeEval{\lpemeta}{\enc(\ctxwold)}{u_1}$ which contradicts the assumption that  $\lpeEval{\lpemeta}{\enc(\ctxwold)}{u_1} = \soi(\adoc(u_1),\ctxwold)$.
\end{proof}
\younes{Anyway, I am still aiming to propose another version of the proof. }




% As a corollary of the previous two propositions, we also see that the sets captured by \ldql are not closed under infinite unions. 


% Let 



 




% 
% The question we want to answer is: for which classes $\classS$ of functions $s$ does there exist an encoding of these functions as triples and a single \lpe $\lpemeta$ 
% 
% 
% given a \caWOLD \ctxwold, can we encode the functions $s$ as triples to be added to the document   can we encode the functions $s$ in the subweb constructions as triples, to  for which classes of functions $s$ is it possible 
% 










\ignore{


To study distribution in \ldql, we will use a simplified version of our goals and assume that with each\footnote{For ``legacy'' documents, the associated link path expression will simply be $\epsilon$, i.e., only include myself.} URI $u$ a link path expression $\lpe(u)$ is associated with intended interpretation that the documents of interest identified by the publisher of the document are those in $\lpeEval{\lpe(u)}{\wold}u$. We will use this in the following way: in case a query agents wants to use information from $u$ to evaluate their query in, and trusts the judgement of the publisher of $u$ they will also include all documents identified by \URIs in $\lpeEval{\lpe(u)}{\wold}u$. 
% , are equally reliable \younes{I think it would be helpful to make this notion clear and agree on a name that we present to the reader. I mean the notion of trust/includes/consider as reliable/... Having a fixed name for it and clearly introduce it to the reader helps us to use it in the rest of the paper uniquely so the reader is not lost.} as $u$ itself and hence that if 
Such situation can occur for instance when a publisher distributes their information over different documents. 
It is important to stress here that \textbf{this assumption is not made in the general framework we propose in \cref{sec:ours}}, but merely serves as a simplification; 
the most important result in this section is that even with this simplification, \ldql cannot deal with distribution of source selection knowledge. In the next session we shall dive more into the ability of \ldql to deal with this fourth property.


For the sake of this section, let us fix
\begin{itemize}
 \item A \WOLD $\wold = \tuple{\docs, \data, \adoc}$
 \item A function $\lpe$ that associates to each $u\in\uris$ a link path expression 
 \item A seed document $u_s$
\end{itemize}
The set $\uris_{result}$ of \URIs the query agent needs to consider for $u_s$ is then: 
\[ \uris_{result}(u_s) = \{u_s\}  \cup \bigcup_{u\in\uris_{result}} \lpeEval{lpe(u)}{\wold}{u}\]
\bart{The distinction between \emph{document} and \emph{uri} (and especially the fact that one cannot go back from doc to uri) is quite annoying}. 


Now, the question we want to answer is whether \ldql, without changing what constitutes a \WOLD, can simulate this. I.e., whether it is possible to \textbf{encode} each link path expression $l$ as a set of triples $\mathit{encode}(l)$ and conceptually \textbf{add} these triples as meta-information to the respective documents such that a single (meta) link path expression evaluates --- over this extended \wold --- to $\uris_{result}$. 

What we show in the rest of this section is
\begin{enumerate}
 \item that in case the link path expressions are extremely simple, such an encoding does exist 
 \item that for slightly more complicated link path expressions, no such encoding can exist, even for this simplified case
\end{enumerate}

\bas{Can we make ``Extremely simple'' and ``slightly more complicated'' more concrete?}

\subsubsection*{For simple path expressions, \ldql \emph{can} simulate distribution}

We start by a simple case where an agents explicitly state what are their \URIs of interest. We use $\uSet(u)$ to denote the set of \URIs determined by $u$. While it seems quite simple to construct an \lpel that simply enumerates all elements in a set, to do it precisely requires some care. The following expression for $\lpel(u)$ has the property that $\lpeEval{\lpel(u)}{\wold}{\uctx} = \uSet(u)$ for any wold \wold  and any context \URI $\uctx$:
\[\lpel(u)= \tuple{?v, SEED\ \uSet(u)\ \tuple{\varepsilon, GRAPH\ ?v\ \{\}}} \]

% \bart{Why is this so complicated? I don't really understand the above expression... Can an explicit enumeration not be simpler in LDQL?} \younes{It appears to be the only \lpel to express direct URIs inclusion, unless I missed some details. In fact, \lpels (more precisely LP) include URIs by matching the underscore operator against triples \textit{in the doc itself}, this leaves \lpels whose semantic doesn't rely on the underscore, namely: \lpels that uses the syntax (?v, q) with q an LDQL query. And LDQL queries have the form (\lpel,P), SEED U q', SEED ?v q', q1 AND/OR q2, $\pi_V$ q. Maybe (\lpel,P) can be used instead by forcing the SPARQL expression to produce the URIs in question, but it is still complex. }

% \younes{trusted by $u$ seems strange to me. Maybe emphasis in the beginning of the paper that we mean by it 'trusted by the agent reachable via $u$' or introduce a notation for agents (for example a function $ag : \uris \rightarrow \mathcal{A}$ that return for an URI its agent, but we should give some sense to agents in this case) }.

Now the encoding we use creates a set of triples using a novel predicate name $\ofinterest$ with the intended interpretation that $(u,\ofinterest,u')$ means that $u'$ is a document identified by $u$.
The encoding of the \lpe of $u$, which serves only to identify the documents in $include(u)$ can then be done by the set of triples 
\[\{\tuple{u,\ofinterest,u'}\mid u'\in include(u)\}.\]

We now claim that the expression \[ e= \tuple{+, trust, \_}^*\] 
can serve to indeed identify all the documents of interest (recursively). This is formalized in the following proposition. 

\begin{proposition}\label{prop:expressible}
 Let \wold be a WOLD that does not use  \ofinterest and let $\uSet(u)$ be a set of \URIs for every $u\in\uris$. 
 Let $\wold'$ be the extension of $\wold$ with 
 \[\data'(d) = \data(d)\cup \{ \tuple{u,\ofinterest,u'}\mid \adoc(u)=d\land u'\in include(u)\}.\]
 As before, let $\uris_{result}(u_s)$ denote the set of \URIs $ \{u_s\}\cup \{ u'\mid u' \in \uSet(u)\land u \in \uris_{result}\}$. In that case, for every $u_s$, we have that 
%  \[
\[\lpeEval{\tuple{+, trust, \_}^*}{\wold'}{u_s} =  \uris_{result}(u_s).\]
\younes{I propose to add a \WOLD parameter to \ures. this will make the transformation more clear by seeing that \ures uses \wold instead of \wold'.}
\end{proposition}



% 
% 
% And to avoid conflict with what exists already in the \WOLD, we require that $trust$ doesn't occur \todo{define occur in \WOLD} in the \WOLD in question. Note that we use the authoritative \URI (the one we are encoding its \lpe) as subject, this gives a more natural way to read it: $u$ trusts $u_i$.
% 
% Now, we are ready to introduce the (meta) \lpel that will simulate $\uris_{result}$. Namely, let $e$ an \lpedefined as
% 
% \[ e= \tuple{+, trust, \_}^*\] 
% \bart{is LDQL syntx underscore or $-$?} \younes{It is underscore, I checked again.}
% 
% We have that $v\in\uris_{result}(u_s)$ iff $v\in\evaluation{e}{\wold}^{u_s}$ for all $v\in \uris$.
% \begin{proof}[Proof Sketch]
%  Let $u_s$ be any \uri, and let $e$ denote $\tuple{+, \ofinterest, \_}^*$. We will show that $\lpeEval{e}{\wold'}{u_s} =  \uris_{result}(u_s)$. 
%  Now, it is easy to see that $v\in \lpeEval{e}{\wold'}{u_s}$ if and only if $v$ is reachable from $u$ by following e
% \end{proof}


\begin{proof}
% 	We prove the equivalence by showing that $\uris_{result}(u)=\evaluation{e}{\wold}^{u}$ for all $u\in \uris$. Let's first rewrite both formulas to have a clearer equivalence. 
Let $u_s$ be any \uri, and let $e$ denote $\tuple{+, \ofinterest, \_}^*$. We will show that $\lpeEval{e}{\wold'}{u_s} =  \uris_{result}(u_s)$. 





We know that 
\[ \lpeEval{e}{\wold'}{u_s} = \bigcup_{i\in \nat} E_i\] where each 
$E_0 = \lpeEval{\varepsilon}{\wold'}{u_s} = \{u_s\}$ and $E_{i+1}= \bigcup_{v\in E_{i}}\lpeEval{\tuple{+, \ofinterest, \_}}{\wold}{v}$.
Similarly, we see that 
\[\uris_{result}(u) = \bigcup_{i\in \nat} U_i\] with 
$U_0= \{u_s\}$ and $U_{i+1} = \bigcup_{v\in U_i} \uSet(v).$ \younes{the passage to \uSet(v) (from the original \lpel(u) used by \ures) seems premature for me. In the original \ures we used \lpel(v) I think the passage from that to \uSet{v} is not very  clear.} 
Now, this follows immediately from the fact that $\wold$ does not mention $\ofinterest$ and  in $\wold'$, the triples in $\adoc(v)$ that match the \lpel $\tuple{+, \ofinterest, \_}$ in context $v$ are exactly the triples $\tuple{v,\ofinterest,w}$ with $w\in include(v)$.



% the  triples of the form $\triple{v,\ofinterest, w}$ in $\adoc(v)$ are exactly those 
% 
% We will show that for each $i$, $E_i$ and $U_i$ actually coincide by induction. 
% For this, it suffices to show that $\lpeEval{\tuple{+, \ofinterest, \_}}{\wold}{v}=include(v)$ for every $v$. 
% %is defined as $\big
% 
% 
% Rewriting the definition of $\uris_{result}$ 
% 
% 
% % we will show that 
% 
% % Fix $u_s$ throughout this proof. 
% % 	
% 	$\uris_{result}(u)$ has a recursive definition, we want to decompose it into a recurrent sequence: let $\uris_{{result}_0}=\{u\}$ and $\uris_{{result}_i}= \bigcup_{v\in\uris_{{result}_{i-1}}} \evaluation{\lpel(v)}{\wold}^{v}$.
% 	It is easy to see that $\uris_{result}(u)$ can be rewritten as
% 	
% 	\[\uris_{result}(u)=\uris_{{result}_0} \cup \uris_{{result}_1} \cup ... \cup \uris_{{result}_n}\]
% 	
% 	
% 	On the other hand side, $\evaluation{e}{\wold}^{u}$ is defined using the $.^*$ operator, and from the semantic of this latter and of the sequence construction ($\lpel_1/\lpel_2$) we can rewrite $\evaluation{e}{\wold}^{u}$ as 
% 	
% 	\[\evaluation{e}{\wold}^{u}= e_0 \cup e_1 \cup ... \cup e_n\]
% 	
% 	with $e_0= u$ and $e_i= \bigcup_{v\in e_{i-1}} \evaluation{\tuple{+, trust, \_}}{\wold}^{v}$.
% 	
% 
% 	We can already see a similarity between both formulas. We show their equivalence by showing that $e_i=\uris_{{result}_i}$ for all $i\in 0..n$. We do so by induction: the base step is trivial, namely $e_0=\uris_{{result}_0}=u$. Suppose that $e_{i-1}=\uris_{{result}_{i-1}}$ is true, we show that $e_{i}=\uris_{{result}_{i}}$ is also true. 
% 	
% 	By definition $\uris_{{result}_i}= \bigcup_{v\in\uris_{{result}_{i-1}}} \evaluation{\tuple{?v, SEED\ include(v)\ \tuple{\varepsilon, GRAPH\ ?v\ \{\}}}}{\wold}^{v}$, which can be reduced to $\uris_{{result}_i}= \bigcup_{v\in\uris_{{result}_{i-1}}} include(v)$ following the semantics of $SEED\ U$ (with $U$ a set of, \URIs) operator and $\tuple{\varepsilon, GRAPH\ ?v\ \{\}}$. Same for $\uris_{{result}_i}$, we have that each agent $v$ embeds its trusted \URIs as triples of the form $\tuple{+, trust, u_i}$ for each $u_i \in include(v)$, which leads to the fact that $\evaluation{\tuple{+, trust, \_}}{\wold}^{v}= inlude(v)$, and consequently to $e_i= \bigcup_{v\in e_{i-1}} include(v)$. Now, we from the induction supposition we have $e_{i-1}=\uris_{{result}_{i-1}}$ and thus $e_i=\uris_{{result}_{i}}$ which concludes the proof. $\qed$
$\qed$
\end{proof} 


\paragraph{A less simple case} The ideas in Proposition \ref{prop:expressible} can also be extended to a setting where the different data publishing agents can choose, for each \URI of interest $u$, whether to include only $u$, or $u$, \URIs determined by $u$, \URIs determined by these latters... in a recursive manner.
A such extension can be done using two \lpes, one for selecting \URIs without further recursion, and one for \URIs whose determined \URIs are to be included as well, which is the current behavior. Formally, a such extension of \ures can be written as $\ures_{ext}(u)=\brak{u}\cup \lpeEval{\lpeEx_{nr}(u)}{\wold}{u}  \cup \ures(u)$ with $\lpeEx_{nr}(u)$ is an \lpe that has the intended meaning of `\URIs that I won't include their determined \URIs'. 

\ldql can tackle the extended case without difficulty. Namely, we need only combine the added \lpe, which is $\lpeEx_{nr}(u)$, with our existing expression $e$ using the alternation connector . 


%do not have to decide to include all documents of 
%
%\paragraph{Less simple case} We would like to present another use case which can be simulated by \ldql, before we dive into a complicated case. In this use case we give agents more control. We allow agents to state whether to include only the agents they trust, or also include what these laters trust. In other words, each agent would have two sets of \URIs: one for which only the \URIs are trusted, and another set for which \URIs and their preferences are both included. Formally, let $includeU$, 
% }
%
%
%\younes{I think about showing the expressiveness also when dealing with two types of URIs (one that includes doc's content and one that includes doc's subweb). Maybe I wait to see if the size of the paper allows it? }
%\bart{It would be nice if you can write this out as well.
%In practice, the proof will probably not be part of the main body of the paper, but move to some appendix. So length of that is not so important}
%\younes{When I tried to write down this example I found out that it doesn't work. Indeed, $\uris_{result}$ by default includes documents and subwebs (subwebs because of recursivity). If we want to show that \ldql can handle this use case, we want to do it independently from $\uris_{result}$.}


\subsubsection*{For interesting path expressions, \ldql \emph{cannot} simulate distribution}


In this section we tackle a richer use case, where agents have more complex preferences (documents of interest). Before addressing this use case, we shall discuss a specific fragment of \ldql formalism.


\paragraph{The primitive fragment of \ldql}
We know \todo{[cite \ldql]} that every \lpe can be represented using only the operators \starop and $\tuple{?v, q}$ (with $q$ an \ldql query) and the \lpe$\varepsilon$. This allows us to limit our investigation to only \lpes that use these components. As a result, an \lpe construction (without considering the \starop operator) can be of two forms: i) $\varepsilon$, or ii) $\tuple{?v, q}$, with $q$ an \ldql query.

On top of that, by looking at the syntax of \ldql queries, we recognize a recursive pattern of \ldql queries even in the primitive fragment. Precisely, in the construction \tuple{e,P} $e$ can take the form $\tuple{?v, q}$ with $q$ an \ldql query, which triggers the cycle of recursivity.

In the following, \lpes use the primitive fragment of \ldql unless stated differenetly.



\paragraph{\ldql navigation}
From the semantics of \ldql queries, the \sparql \sparqlex graph pattern to be answered is evaluated against some dataset. This latter is obtained from the \URIs returned by the \lpe associated to \sparqlex. We have that for each mapping $\mu$ $\in$ \queryEval{\sparqlex}{}{\dataset}, each object in \img($\mu$) should occur in \dataset. And we could have for some set of seeds $S$ and \lpe$l$ an object $a$ that occurs in \datasetW{\wold}(\lpeEval{l}{\wold}{S}) but not in \datasetW{\wold}. In fact, this observation highlights the ability of \lpes to traverse the \wold, but also indicates that this traversal is performed only by link path expressions and not by \sparql.
In fact, there is two manners in which \lpes can achieve this traversal, namely
\begin{itemize}
	\item \lpes of the form $\tuple{?v, q_1\ldqlAND q_2}$ with
	\begin{itemize}
		\item $q_2=\ldqlSeed\ ?x\ q_2'$ with $q_2'$ mentions $?v$,
		\item $q_1$ produces a mapping $\mu$ with $\mu(?x) \in \uris$.
	\end{itemize}
	
	

	this case covers the case $l/l'$ where $l$ and $l'$ are \lpes,
	\item \lpes of the form $l^*$ with $l$ an \lpe.
\end{itemize}


Before showing the limitation of these two queries, we shall present a particular property of \lpes.

\begin{lemma}
	For an \lpe$l$ that doesn't use the \starop operator, $l$ should use at least $n$ expressions of the form $\tuple{?v, q_1 \ldqlAnd  \ldqlSeed\ ?x q_2}$ to get a \URI that is separated by $n$ links from $S$. \todo{define separated + link}
\end{lemma}

\begin{proof}
	Let $l$ an \lpe equals to $\tuple{?v, q_1 \ldqlAnd  \ldqlSeed\ ?x q_2}$ with $q_1$ and $q_2$ \ldql queries that don't use the \starop nor the $\ldqlSeed$ operator.
	
	 Since $q_1$ doesn't use the \starop nor the $\ldqlSeed$ operator, every mapping produced by $q_1$ has its \URIs values separated by $0$ links from the seeds set. And from the semantics of $\ldqlSeed\ ?x q$ queries and the fact that $?x$ is bound (to a \URI of distance 0 from the seeds set) by some mapping from $q_1$, we have that every mapping produced by $q_2$ has its \URIs values separated by at most $1$ links from the seeds set. 
	 
	 
	 Now Consider a general \lpe$l=\tuple{?v, q_1 \ldqlAnd  \ldqlSeed\ ?x q_2}$ with the required conditions of traversal \todo{refer to these conditions}, and suppose (WLOG) that $q_2$ doesn't use the $\ldqlSeed$ operator. Following the result in the previous paragraph, and by induction on $q_1$, each occurrence of the $\ldqlSeed$ operator increases the distance of the resultant \URIs by at most 1. Hence, each \URI produced by $l$ is separated at most $n$ links, where $n$ is the number of $\ldqlSeed$ operators in $q_1$ plus 1. $\qed$
\end{proof}
\younes{this lemma is to be used to show that the general \lpe is bound by the size of \docs minus one if it uses SEED operator. An example to show this is a \WOLD with a chain of documents without cycles.}
\todo{seed query size}

We now show the limitation of the \starop. As an example we consider a \WOLD \wold with four documents $\adoc(u_1),..,\adoc(u_4)$ whose preferences are 


\begin{itemize}
	\item $\lpel(u_1) = \varepsilon\lpeOr \tuple{+,\pred{foaf:friend},\_} \lpeOr \tuple{+,\pred{foaf:friend},\_}/\tuple{+,\pred{foaf:friend},\_}$: myself, friends of mine, and friends of my friends,
	\item $\lpel(u_2)=\varepsilon\lpeOr \tuple{+,\pred{foaf:colleagues},\_} \lpeOr \tuple{+,\pred{foaf:friend},\_}/\tuple{+,\pred{foaf:friend},\_}$: myself, colleages of mine, and colleages of my colleages,
	\item $\lpel(u_3)=\varepsilon$ : myself,
	\item $\lpel(u_4)=\varepsilon$ : myself,
\end{itemize}


and let \wold be such that $\docs=\brak{\adoc(u_1)..\adoc(u_4)}$ and 

\begin{itemize}
	\item $\data(\adoc(u_1))= \brak{\tuple{u_1,\pred{foaf:friend},u_2}}$,
	\item $\data(\adoc(u_2))= \brak{\tuple{u_2,\pred{foaf:colleague},u_3}}$,
	\item $\data(\adoc(u_3))= \brak{\tuple{u_3,\pred{foaf:friend},u_4}, \tuple{u_3,\pred{foaf:colleage},u_5}}$.
\end{itemize}
\todo{figure}

The content of documents \adoc($u_4$) and \adoc($u_5$) is not important for our illustration. 
The preferences of the documents give the following determined \URIs

\begin{lstlisting}[caption={Determined \URIs of each agent},captionpos=b,label={listing:subwebs}]
	
			u_1's determined URIs are {u_1,u_3,u_4}
			u_2's determined URIs are {u_2,u_3,u_5}
			u_3's determined URIs are {u_3}
	
\end{lstlisting}


Note that the \URIs present in some document are not necessarily determined by that document. For instance, $\adoc(u_3)$ contains the \URI $u_4$, but this latter is not determined by $u_3$.


Following the same strategy as the previous section (proposition \ref{prop:expressible}) we want to embed the preferences of each agent in its authoritative document. But as we will see, there is no encoding that allows to get to the desired results. Therefore, we keep such encoding abstract and we show that there is no $\lpe$ that gives rise to the wanted result (Listing \ref{listing:subwebs}), no matter what encoding we are using. 

We set \wold' to be the \WOLD obtained from \wold in which the preferences of different agents are embedded into their documents. In other words, for each agent $u_i$ we have $\data'(u_i)=\data(u_i) \cup \encode(\lpe(u_i))$ with \encode a function produce a triple representation of an \lpe. That being said    %\brak{\tuple{p_{s_1}, p_{p_1}, p_{o_1}}


\younes{Note that the proposition refers to the subwebs stated in the Listing as English sentences rather than using \ures. This is because \ures cannot generate those results. Maybe we will have to change it to not have it introduced for only the first part (expressiveness).}

\begin{proposition}
	There exist no \lpe$e$ whose evaluation in \wold' gives rise to the results in Listings \ref{listing:subwebs}.
\end{proposition}

\begin{proof}
	We proceed in two steps. In a first time we prove the case where $e$ doesn't use the \starop, then we tackle the general case. In both cases we suppose wlog that $e$ doesn't mention the \URIs $u_4$ and $u_5$ nor the predicates $\pred{foaf:friend}$ or $\pred{foaf:colleage}$. 
	
	
	
	Suppose $e$ doesn't use the \starop operator, we know that \lpeEval{e}{\wold'}{u_1} doesn't contain $u_3$\footnote{recall that $e$ uses only the construction \tuple{?v, P}, the operator \starop and the \lpe$\varepsilon$.}, since whatever is the form of $e$ it is evaluated on \data(\adoc($u_1$)) which doesn't contain the \URI $u_3$. And thus $e$ cannot get the set of \URIs determined by $u_1$. This suggests that the usage of the \starop is imperative in order to be get the $u_3$.
	
	Now, suppose that $e$ uses the \starop operator. There might be several instances of that operator, we are particularly interested in the instance of this operator that leads to $u_3$. Let $e_s^*$ be that instance, from the semantics of the \starop operator we recognize that  \lpeEval{e_s^*}{\wold'}{u_1} yields \lpeEval{e_s^*}{\wold'}{u_2}. But then, because
	\younes{two ideas. 1) the symmetry argument, 2) the unstoppability of \starop operator.}
	
\end{proof}







-------------------------------------------------------------
----------------------- SERVICE -------------------------------
-------------------------------------------------------
\begin{center}
	\begin{tabular}{l l}
		$\data(d_1)$&=$\brak{(u_1,friend,u_2)}$\\
		$\data(d_2)$&=$\brak{(u_2,colleague,{u_2}_c), (u_2,friend,u_3)}$\\
		$\data(d_3)$&=$\brak{(u_3,colleague,{u_3}_c), (u_3,friend,{u_3}_f)}$\\
	%	$\data(d_4)$&=$\brak{(u_4,colleague,{u_4}_c), (u_4,friend,{u_4}_f)}$\\
	\end{tabular}
\end{center}


Moreover, these are the (informal) agents' construction rules 

\begin{itemize}
	\item $\lpel(u_1) = \varepsilon\lpeOr \tuple{+,\pred{foaf:friend},_} \lpeOr \tuple{+,\pred{foaf:friend},_}/\tuple{+,\pred{foaf:friend},_}$ : myself, friends of mine, and friends of my friends,
	\item $\lpel(u_2)$ : myself and my colleagues,
	\item $\lpel(u_3)$ : myself ($\varepsilon$),
\end{itemize}

In this scenario, the subweb of $d_1$ is $\uris_{result}(u_1)= \brak{u_1, u_2, u_3}$. Namely, what we are looking for is a general \lpe$e$ such that:

\begin{equation} \label{targetSWsWithlpe}
	\begin{tabular}{l l}
		$\lpeEval{e}{\wold}{u_1}$&=\brak{u_1, u_2, u_3}\\
		$\lpeEval{e}{\wold}{u_2}$&=\brak{u_2, {u_2}_c}\\
		$\lpeEval{e}{\wold}{u_3}$&=\brak{u_3}\\
	%	$\lpeEval{e_c}{\wold}{u_4}$&=\brak{u_4}\\
	\end{tabular}
\end{equation}

Before discussing the existence of $e$, let us analysis the structure of \lpes.


\begin{claimN}\label{claimSparql10Navigation}
	For $P$ a \sparql (1.0) expression, if $\mu \in \queryEval{P}{}{dataset_\wold(u)}$ then $img(\mu)$ should occur \todo{define occur} in some graph of $dataset_\wold(u)$.
\end{claimN}


\paragraph{restricted \lpe} Now, getting back to $e$. Indeed, $e$ rely on \sparql which has a high expressiveness, this makes the non existence of $e$ non obvious. Therefore, we decompose the task of proving the non existence of $e$ into smaller pieces. First, we consider a specific form of $e$ where we don't use the \starop operator. Let $e_{ns}$ a family of \lpes obtained from a restriction of $e$ where the \starop operator isn't used.

\begin{lemma}
	there exist no $e_{ns}$ that generates the results in Equation \ref{targetSWsWithlpe}.
\end{lemma}


\begin{proof}
	Consider the most basic $\lpel$: i) $\varepsilon$ clearly can't achieve the goal (equation \ref{targetSWsWithlpe}), and ii) we have $\tuple{?v, q}$ which we tackle by induction on the structure of $q$. The base case of the proof starts from the most basic form of $q$, which is $\tuple{\varepsilon, P}$. From the semantic of LDQL we have 
	
	
	{\renewcommand{\arraystretch}{1.5}
		\begin{tabular}{l l}
			
			$\lpeEval{\tuple{?v, \tuple{\varepsilon, P}}}{\wold}{u_1}$&$= \brak{u\in \uris \mid \exists \mu \in \lpeEval{\tuple{\varepsilon, P}}{\wold}{u_1},\ s.t.\ u=\mu(?v)}$\\
			&$=\brak{u\in \uris \mid \exists \mu \in \queryEval{P}{}{dataset_\wold(\lpeEval{\varepsilon}{\wold}{u_1})},\ s.t.\ u=\mu(?v)}$\\
			&$=\brak{u\in \uris \mid \exists \mu \in \queryEval{P}{}{dataset_\wold(u_1)},\ s.t.\ u=\mu(?v)}$
		\end{tabular}
	}

We see from the previous formulas that the result is mainly computed using $\queryEval{P}{}{dataset_{\wold(u_1)}}$. And based on claim \ref{claimSparql10Navigation}, $\queryEval{P}{}{dataset_{\wold(u_1)}}$ cannot be used to get the wanted results since ${u_3}$ doesn't occur in  $dataset_{\wold(u_1)}$, and thus cannot be in its subweb (the subweb of $u_1$). 

Now, assume $q$ and $q_2$ such that neither $\tuple{?v, q}$ nor $\tuple{?v, q_2}$ can achieve the results in Equation \ref{targetSWsWithlpe}. We show that the other constructions of \ldql queries cannot achieve the results in Equation \ref{targetSWsWithlpe}:

\begin{itemize}
	\item for the case $\tuple{?v, SEED\ U\ q}$: based on the semantics of \ldql this is always equal to $\queryEval{q}{\wold}{U}$ regardless of the \URI on which it is evaluated. That said, it generates exactly the same set of \URIs for all agents, and clearly cannot be used to achieve the results in Equation \ref{targetSWsWithlpe}.
	
	\item for the case $\tuple{?v, SEED\ ?v'\ q}$: based on the semantics of \ldql this will evaluate $q$ on all existing agents, which again generates exactly the same set of \URIs for all agents, and clearly cannot be used to achieve the results in Equation \ref{targetSWsWithlpe}.
	
	\item for the case $\tuple{?v,qANDq_2}$: \younes{this is not obvioous. to be reviewed.}
	\item for the case $\tuple{?v,qUNIONSq_2}$: \younes{this is not obvioous. to be reviewed.}
	\item for the case $\tuple{?v, \pi_V q}$: we have two cases: i) $?v \not\in V$ which gives always the empty set and thus cannot achieve the results in Equation \ref{targetSWsWithlpe}, and ii) $?v \in V$: in this case $\tuple{?v, \pi_V q}\equiv \tuple{?v, q}$ and thus it cannot achieve the wanted goal. $\qed$ 
	
\end{itemize}


\end{proof}

\paragraph{Federated SPARQL} Nevertheless, there is an exception to the previous lemma. Federated SPARQL \cite{cite} can get results outside the graph at input through the directive SERVICE. This means that Claim \ref{claimSparql10Navigation} no longer holds. However, the evaluation of an expression $SERVICE\ ?X\ P$ is infeasible unless $?X$ is bound to a finite set of variables. This condition ($?X$ being bound) is satisfied if a certain property of \emph{boundedness} is satisfied, but agreement on the notion of \emph{boundedness} doesn't exist yet \todo{citation}: roughly, for $SERVICE\ ?X\ P$ to be computable, the idea is that $?X$ should be guaranteed to be bound by an expression outside $P$. In such a way, we would evaluate that expression before evaluating $SERVICE\ ?X\ P$.

Let's get more formal by focusing on the semantic of $SERVICE$ operator. A such semantic has been proposed in \cite{citation} as follow: let $ep$ (for endpoint) a function that maps a \URI to the dataset that is associated with it, and use $graph(n, ds)$ to access to the graph named $n$ in the dataset $ds$. Then if $P$ is $(SERVICE\ c\ P_1)$ with $c\in \uris \cup \vars$, then

\[
\queryEval{P}{G}{DS}=\left\{ \begin{array}{l l}
	\queryEval{P_1}{graph(def, ep(c))}{ep(c)}& if\ c\in \uris\\
	\emptyset& if\ c\in \uris\backslash dom(ep)\\
	\{\mu\cup \mu_c \mid \exists s\in dom(ep): \mu_c=\{c\mapsto s\}, &\\
	\mu \in \queryEval{P_1}{graph(def, ep(s))}{ep(s)},\ and\ \mu_c \textasciitilde{} \mu \}& if\ c\in \vars\\
\end{array}\right.
\]

For the third case, as discussed in \cite{federated} about $SERVICE$ boundedness, $c$ should be (\emph{strongly}) bound in some expression outside $P$: that is, $\mu_c$ should be guaranteed to exist prior to the evaluation of $P$.

Now, we get back to our discussion about $\tuple{?v, \tuple{\varepsilon, P}}$. We first tackle a concrete case using $SERVICE$ to make the behavior of $SERVICE$ more clear, then we show that this latter is not sufficient to express the subweb of $u_1$. Suppose $P$ uses a sub expression of the form $SERVICE\ ?X\ P_1$ so it can fetch the \URI $u_3$ from $d_2$ (by binding $?X$ to $u_2$). Now we slightly alter the subweb of $u_2$ in order to illustrate the idea: assume that $\lpel(u_1)$ expresses `myself, my friend, friends of my friends, and friends of my friends' friends', this generates the same subweb as before in addition to ${u_3}_f$.

We argue that, another expression $SERVICE\ ?Y\ P_2$ should be present in either $P_1$ or $P$ in order for $e_{ns}$ to fetch the \URI ${u_3}_f$ from $d_3$ (by binding $?Y$ to $u_3$). In the contrary (if neither $P_1$ nor $P$ has another sub expression of the form $SERVICE\ ?Y\ P_2$), ${u_3}_f$ cannot be fetched. 

\begin{claimN}
	If $e_{ns}=\tuple{?v, \tuple{\varepsilon, P}}$ uses only one expression of the form $SERVICE\ ?X\ P_1$, it is impossible for $e_{ns}$ to get ${u_3}_f$.
\end{claimN}

\begin{proof}
	First, from the boundedness of $SERVICE$ we have that: to evaluate $SERVICE\ ?X\ P_1$, $?X$ should be already bound in $P$ to some \URI $c$, and from Claim \ref{claimSparql10Navigation} $c$ cannot be $u_3$ (which leads to ${u_3}_f$) because there is no other $SERVICE$ directive in $P$. In fact, all what $?X$ can be bound to is $u_2$. This gets us to the second case.
	
	Suppose now that $?X$ is bound to $u_2$, in this case: $P_1$ will be evaluated on $ep(u_2)$, which again based on Claim \ref{claimSparql10Navigation}, cannot generate ${u_3}_f$ since this latter doesn't occur in $ep(u_2)$. $\qed$
\end{proof}

Now, suppose that $e_{ns}$ uses SPARQL 1.1 (Federated SPARQL). For the next Lemma, we define the size of an \lpel by the number of $SERVICE\ ?X\ P$ expressions.

\begin{lemma}\label{lpeNsUnexist}
	$e_{ns}$ cannot exist independently from the \WOLD in question. And the size of $e_{ns}$ is bound by the size of the \WOLD in question.
\end{lemma}

\begin{proof}
	In fact, one can easily see that to get from a document $d$ to a document $q$ that are separated by $n$ links \todo{define link: getting from a document to another following a URI from the first} we have to use the expression $SERVICE\ ?X\ P$ $n$ times, one time for each link. That said, to construct $e_{ns}$ for some $u$, we need to know in advance the farthest document $v$ to be included in the subweb of $u$. This requires us to know the \WOLD in question (and the subweb of $u$) in advance, hence $e_{ns}$ cannot exist independently from the \WOLD in question. 
	
	For the size of $e_{ns}$, we can see that $n$ can be equal to the number of documents in the \WOLD minus 1: take a \WOLD \wold where i) each document is linked exactly to one document, ii) no two documents are linked to each other, and iii) each document should have exactly one outgoing link and one incoming link, except two documents $d$ and $q$: $d$ has only an outgoing link and $q$ has only an incoming link. Now suppose that the subweb of $d$ contains $q$, in this case $u$ needs an $e_{ns}$ of size $n-1$ in order to get $q$, where $n$ is the number of documents in \wold. $\qed$
\end{proof}

	\younes{So $e_{ns}$ can exist. What can't be possible is the existence of $e_{ns}$ independtly of \wold: maybe this can be reformulated as $e_{ns}$ is not declarative?. And a second point is the size of $e_{ns}$ which is very big and which is a consequence of the first point.
	
I think the important block in this proof is the first part where it is said 'one can easily see that': we are relying a bit on the reader's intuition.}


\paragraph{The star operator} We now consider $e$ with the star operator, that is $e=e_{ns}^*$. Recall that we want $e$ such that Equation \ref{targetSWsWithlpe} holds. We shall state directly our result regarding the non existence of $e$.

\begin{lemma}
	There is no $e$ that simulates $\uris_{result}$.
\end{lemma}

\begin{proof}
	We show the above lemma by providing a case for  $\uris_{result}$ that $e$ cannot simulate. Consider the subweb of $u_1$ in Equation \ref{targetSWsWithlpe} which is the result of getting the friends of $u_1's$ friends. Suppose $e$ exists, we get $\lpeEval{e}{\wold}{u_1}$=$\lpeEval{e_{ns}^*}{\wold}{u_1}$. By definition we have that $\lpeEval{\varepsilon}{\wold}{u_1}, \lpeEval{e_{ns}}{\wold}{u_1}, \lpeEval{e_{ns}/e_{ns}}{\wold}{u_1} \in \lpeEval{e}{\wold}{u_1}$. For the first case, we have that $\lpeEval{\varepsilon}{\wold}{u_1}=u_1$. For the rest we discuss two possibilities
	
	\begin{itemize}
		\item $e_{ns}$ doesn't use the $SERVICE$ directive which leads to $\lpeEval{e_{ns}}{\wold}{u_1}=\brak{u_2}$ (or the empty set which is a trivial case):
		
		In this case we will have the second iteration of the expression ($\lpeEval{e_{ns}/e_{ns}}{\wold}{u_1}$) equals to $\lpeEval{e_{ns}}{\wold}{u_2}$. Now, from the (informal) subweb of $u_2$ we know that $\lpeEval{e_{ns}}{\wold}{u_2}$ should return ${u_2}_c$ and not $u_3$, but from the subweb of $u_1$ we have that $\lpeEval{e_{ns}/e_{ns}}{\wold}{u_1}$ should return $u_3$ which is a contradiction.
		
		\item $e_{ns}$ uses the $SERVICE$ directive where we consider two cases
		\begin{itemize}
				\item case 1: one iteration of $e$ gets all the required results, that is \lpeEval{e_{ns}}{\wold}{u_1}= \brak{u_2, u_3}. In this case we refer to the previous proof (Lemma \ref{lpeNsUnexist}) about the existence of $e_{ns}$,
				\item case 2: one iteration of $e$ is not sufficient to get the required results, that is i) \lpeEval{e_{ns}}{\wold}{u_1}= \brak{u_2}, ii) \lpeEval{e_{ns}}{\wold}{u_1}=\brak{u_3}, or iii) \lpeEval{e_{ns}}{\wold}{u_1}= $\emptyset$. The latter is clearly unable to get the wanted results. In (ii) we would have \lpeEval{e_{ns}}{\wold}{u_3} in the second iteration which is equalt to $\emptyset$ based on $u_3$'s subweb, and thus (ii) doesn't get the required subweb for $u_1$ (namely, it misses $u_2$). Lastly, (i) would have \lpeEval{e_{ns}}{\wold}{u_2} in the second iteration, which based on $u_2$'s subweb doesn't include $u_3$ (which should present in $u_1$ subweb) and thus doesn't cover the correct subweb. $\qed$
		\end{itemize}
			
	\end{itemize}



\end{proof}
}

